Dynamical behavior of a time-delayed infectious disease model with a non-linear incidence function under the effect of vaccination and treatment

When an infectious disease propagates throughout society, the incidence function may rise at first due to an increase in pathogenicity and then decrease due to inhibitory effects until it reaches saturation. Effective vaccination and treatment are very helpful for controlling the effects of such infectious diseases. To analyze the impacts of these diseases, we proposed a new compartmental model with a generalized non-linear incidence function, vaccination function, and treatment function, along with time delays in the respective functions, which show how its monotonic features influence the stability of the model. Fundamental properties of a model, such as positivity, boundedness, and the existence of equilibria, are examined in this work. The basic reproduction number has been computed, and correlative studies for local stability in view of the basic reproduction number have been examined at the disease-free and endemic equilibrium points. A delay-independent global stability result has been established, and to be more precise, we explicitly derived the result on global stability by restricting delay parameters within a very specific range. Furthermore, numerical simulations and some examples based on COVID-19 real-time data are pointed out to emphasize the significance of how the disease's dynamical behavior is characterized by various functions for controlling the spread of disease in a population and to justify the mathematical conclusions.

==> Citations.tex <==


@article{rao2015dynamic,
title={A dynamic model for infectious diseases: The role of vaccination and treatment},
author={Rao, P Raja Sekhara and Kumar, M Naresh},
journal={Chaos, Solitons \& Fractals},
volume={75},
pages={34--49},
year={2015},
publisher={Elsevier}
}
	
@book{rao2013dynamic,
title={Dynamic models of infectious diseases},
author={Rao, Vadrevu Sree Hari and Durvasula, Ravi},
volume={1},
year={2013},
publisher={Springer}
}
@article{KABIR2019118,
title = {Analysis of SIR epidemic model with information spreading of awareness},
journal = {Chaos, Solitons \& Fractals},
volume = {119},
pages = {118-125},
year = {2019},
issn = {0960-0779},
doi = {https://doi.org/10.1016/j.chaos.2018.12.017},
url = {https://www.sciencedirect.com/science/article/pii/S0960077918303898},
author = {K.M. Ariful Kabir and Kazuki Kuga and Jun Tanimoto}
}
@article{rao2019predictive,
author = {Rao, P Raja Sekhara and Ratnam , K Venkata and Mushnuri, Sita Rama},
year = {2019},
month = {01},
pages = {128-139},
title = {Predictive dynamics of infectious diseases-a new technique },
volume = {15},
journal = {World Journal of Modelling and Simulation}
}
@article{DaCosta2019ConditionersOT,
title={Conditioners of the infectious diseases dynamics},
author={Anderson Luiz Pena Da Costa and Orlando Alves Rodrigues Neto and A C T Silva-J{\'u}nior},
journal={Estaç{\~a}o Cient{\'i}fica (UNIFAP)},
  year={2019}
}
@article{Zaman2017,
author = {Zaman, Gul and Jung, Il Hyo and Torres, Delfim F. M. and Zeb, Anwar},
year = {2017},
month = {12},
pages = {1-1},
title = {Mathematical Modeling and Control of Infectious Diseases},
volume = {2017},
journal = {Computational and Mathematical Methods in Medicine},
doi = {10.1155/2017/7149154}
}
@article{Hoertel2020,
author = {Hoertel, Nicolas and Blachier, Martin and Blanco, Carlos and Olfson, Mark and Massetti, Marc and Rico, Marina and Limosin, Frédéric and Leleu, Henri},
year = {2020},
month = {09},
pages = {1-5},
title = {A stochastic agent-based model of the SARS-CoV-2 epidemic in France},
volume = {26},
journal = {Nature Medicine},
doi = {10.1038/s41591-020-1001-6}
}
@article{article2,
author = {Anand, Monalisa and Danumjaya, P. and Rao, P.},
year = {2023},
month = {03},
pages = {346-369},
title = {A nonlinear mathematical model on the Covid-19 transmission pattern among diabetic and non-diabetic population},
volume = {210},
journal = {Mathematics and Computers in Simulation},
doi = {10.1016/j.matcom.2023.03.016}
}

@article{weitz2015modeling,
  title={Modeling post-death transmission of Ebola: challenges for inference and opportunities for control},
  author={Weitz, Joshua S and Dushoff, Jonathan},
  journal={Scientific reports},
  volume={5},
  number={1},
  pages={1--7},
  year={2015},
  publisher={Nature Publishing Group}
}
@article{article1,
author = {Li, Mingming and Liu, Xianning},
year = {2014},
month = {02},
pages = {Article ID 131257, 7 pages},
title = {An SIR Epidemic Model with Time Delay and General Nonlinear Incidence Rate},
volume = {2014},
journal = {Abstract and Applied Analysis},
doi = {10.1155/2014/131257}
}
@article{article7,
author = {Tyagi, Swati and Martha, s and Abbas, Syed and Debbouche, Amar},
year = {2021},
month = {03},
pages = {110707},
title = {Mathematical modeling and analysis for controlling the spread of infectious diseases},
volume = {144},
journal = {Chaos Solitons \& Fractals},
doi = {10.1016/j.chaos.2021.110707}
}
@article{LEE2016118,
title = {A dynamic compartmental model for the Middle East respiratory syndrome outbreak in the Republic of Korea: A retrospective analysis on control interventions and superspreading events},
journal = {Journal of Theoretical Biology},
volume = {408},
pages = {118-126},
year = {2016},
issn = {0022-5193},
doi = {https://doi.org/10.1016/j.jtbi.2016.08.009},
url = {https://www.sciencedirect.com/science/article/pii/S0022519316302430},
author = {Jonggul Lee and Gerardo Chowell and Eunok Jung}
}
@article{ahn2018investigation,
  title={Investigation of nonlinear epidemiological models for analyzing and controlling the MERS outbreak in Korea},
  author={Ahn, Inkyung and Heo, Seongman and Ji, Seunghyun and Kim, Kyung Hyun and Kim, Taehwan and Lee, Eun Joo and Park, Jooyoung and Sung, Keehoon},
  journal={Journal of Theoretical Biology},
  volume={437},
  pages={17--28},
  year={2018},
  publisher={Elsevier}
}
@book{perko2013differential,
  title={Differential equations and dynamical systems},
  author={Perko, Lawrence},
  volume={7},
  year={2013},
  publisher={Springer Science \& Business Media}
}
@article{BERETTA201887,
title = {A mathematical model for malaria transmission with asymptomatic carriers and two age groups in the human population},
journal = {Mathematical Biosciences},
volume = {300},
pages = {87-101},
year = {2018},
issn = {0025-5564},
doi = {https://doi.org/10.1016/j.mbs.2018.03.024},
url = {https://www.sciencedirect.com/science/article/pii/S0025556417304893},
author = {Edoardo Beretta and Vincenzo Capasso and Dario G. Garao},
}
@article{martorano2015equilibrium,
  title={Equilibrium analysis of a yellow fever dynamical model with vaccination},
  author={Martorano Raimundo, Silvia and Amaku, Marcos and Massad, Eduardo},
  journal={Computational and mathematical methods in medicine},
  volume={2015},
  year={2015},
  publisher={Hindawi}
}
@article{TIAN201131,
title = {Global stability for cholera epidemic models},
journal = {Mathematical Biosciences},
volume = {232},
number = {1},
pages = {31-41},
year = {2011},
issn = {0025-5564},
doi = {https://doi.org/10.1016/j.mbs.2011.04.001},
url = {https://www.sciencedirect.com/science/article/pii/S0025556411000654},
author = {Jianjun Paul Tian and Jin Wang},
}
@article{Dumont2011,
author = {Dumont, Yves and Tchuenche, Michel},
year = {2011},
month = {10},
pages = {809-54},
title = {Mathematical studies on the sterile insect technique for the Chikungunya disease and Aedes albopictus},
volume = {65},
journal = {Journal of mathematical biology},
doi = {10.1007/s00285-011-0477-6}
}
@article{LIU20153194,
title = {Application of control strategies to a seasonal model of chikungunya disease},
journal = {Applied Mathematical Modelling},
volume = {39},
number = {12},
pages = {3194-3220},
year = {2015},
issn = {0307-904X},
doi = {https://doi.org/10.1016/j.apm.2014.10.035},
url = {https://www.sciencedirect.com/science/article/pii/S0307904X14005198},
author = {Xinzhi Liu and Peter Stechlinski},
}
@article{Esteva1999,
author = {Esteva, Lourdes and Vargas, Cristobal},
year = {1999},
month = {04},
pages = {220-40},
title = {A model for dengue disease with variable human population},
volume = {38},
journal = {Journal of mathematical biology},
doi = {10.1007/s002850050147}
}
@article{Mapder2019,
    doi = {10.1371/journal.pcbi.1006668},
    author = {Mapder, Tarunendu AND Clifford, Sam AND Aaskov, John AND Burrage, Kevin},
    journal = {PLOS Computational Biology},
    publisher = {Public Library of Science},
    title = {A population of bang-bang switches of defective interfering particles makes within-host dynamics of dengue virus controllable},
    year = {2019},
    month = {11},
    volume = {15},
    url = {https://doi.org/10.1371/journal.pcbi.1006668},
    pages = {1-24},
}
@article{ZHU2019115,
title = {A time-periodic dengue fever model in a heterogeneous environment},
journal = {Mathematics and Computers in Simulation},
volume = {155},
pages = {115-129},
year = {2019},
note = {International Conference on Mathematical Modeling and Computational Methods in Science and Engineering},
issn = {0378-4754},
doi = {https://doi.org/10.1016/j.matcom.2017.12.008},
url = {https://www.sciencedirect.com/science/article/pii/S0378475417304007},
author = {Min Zhu and Yong Xu},
}
@article{de2021dynamics,
  title={Dynamics of epidemics: Impact of easing restrictions and control of infection spread},
  author={de Souza, Silvio LT and Batista, Antonio M and Caldas, Iber{\^e} L and Iarosz, Kelly C and Szezech Jr, Jos{\'e} D},
  journal={Chaos, Solitons \& Fractals},
  volume={142},
  pages={110431},
  year={2021},
  publisher={Elsevier}
}
@article{LIN2020211,
title = {A conceptual model for the coronavirus disease 2019 (COVID-19) outbreak in Wuhan, China with individual reaction and governmental action},
journal = {International Journal of Infectious Diseases},
volume = {93},
pages = {211-216},
year = {2020},
issn = {1201-9712},
doi = {https://doi.org/10.1016/j.ijid.2020.02.058},
url = {https://www.sciencedirect.com/science/article/pii/S120197122030117X},
author = {Qianying Lin and Shi Zhao and Daozhou Gao and Yijun Lou and Shu Yang and Salihu S. Musa and Maggie H. Wang and Yongli Cai and Weiming Wang and Lin Yang and Daihai He},
}
@article{giordano2020modelling,
  title={Modelling the COVID-19 epidemic and implementation of population-wide interventions in Italy},
  author={Giordano, Giulia and Blanchini, Franco and Bruno, Raffaele and Colaneri, Patrizio and Di Filippo, Alessandro and Di Matteo, Angela and Colaneri, Marta},
  journal={Nature medicine},
  volume={26},
  number={6},
  pages={855--860},
  year={2020},
  publisher={Nature Publishing Group}
}
@article{NDAIROU2021110652,
title = {Fractional model of COVID-19 applied to Galicia, Spain and Portugal},
journal = {Chaos, Solitons \& Fractals},
volume = {144},
pages = {110652},
year = {2021},
issn = {0960-0779},
doi = {https://doi.org/10.1016/j.chaos.2021.110652},
url = {https://www.sciencedirect.com/science/article/pii/S0960077921000059},
author = {Faïçal Ndaïrou and Iván Area and Juan J. Nieto and Cristiana J. Silva and Delfim F.M. Torres},
}
@article{hethcote1989epidemiological,
  title={An epidemiological model with a delay and a nonlinear incidence rate},
  author={Hethcote, Herbert W and Lewis, Mark A and Van Den Driessche, P},
  journal={Journal of mathematical biology},
  volume={27},
  number={1},
  pages={49--64},
  year={1989},
  publisher={Springer}
}
@article{COOPER2020110298,
title = {Dynamic tracking with model-based forecasting for the spread of the COVID-19 pandemic},
journal = {Chaos, Solitons \& Fractals},
volume = {139},
pages = {110298},
year = {2020},
issn = {0960-0779},
doi = {https://doi.org/10.1016/j.chaos.2020.110298},
url = {https://www.sciencedirect.com/science/article/pii/S0960077920306949},
author = {Ian Cooper and Argha Mondal and Chris G. Antonopoulos},
}
@article{WEINSTEIN2020132633,
title = {Analytic solution of the SEIR epidemic model via asymptotic approximant},
journal = {Physica D: Nonlinear Phenomena},
volume = {411},
pages = {132633},
year = {2020},
issn = {0167-2789},
doi = {https://doi.org/10.1016/j.physd.2020.132633},
url = {https://www.sciencedirect.com/science/article/pii/S016727892030453X},
author = {Steven J. Weinstein and Morgan S. Holland and Kelly E. Rogers and Nathaniel S. Barlow},
}
@article{prodanov2020analytical,
  title={Analytical parameter estimation of the SIR epidemic model. Applications to the COVID-19 pandemic},
  author={Prodanov, Dimiter},
  journal={Entropy},
  volume={23},
  number={1},
  pages={59},
  year={2020},
  publisher={MDPI}
}
@article{scherer2002mathematical,
  title={Mathematical models of vaccination},
  author={Scherer, Almut and McLean, Angela},
  journal={British medical bulletin},
  volume={62},
  number={1},
  pages={187--199},
  year={2002},
  publisher={Oxford University Press}
}
@article{KUDRYASHOV2021466,
title = {Analytical features of the SIR model and their applications to COVID-19},
journal = {Applied Mathematical Modelling},
volume = {90},
pages = {466-473},
year = {2021},
issn = {0307-904X},
doi = {https://doi.org/10.1016/j.apm.2020.08.057},
url = {https://www.sciencedirect.com/science/article/pii/S0307904X20304984},

author = {Nikolay A. Kudryashov and Mikhail A. Chmykhov and Michael Vigdorowitsch},
}

@article{HUPPERT2013999,
title = {Mathematical modelling and prediction in infectious disease epidemiology},
journal = {Clinical Microbiology and Infection},
volume = {19},
number = {11},
pages = {999-1005},
year = {2013},
issn = {1198-743X},
doi = {https://doi.org/10.1111/1469-0691.12308},
url = {https://www.sciencedirect.com/science/article/pii/S1198743X14630019},
author = {A. Huppert and G. Katriel},
}
@article{opatowski:hal-02089219,
  TITLE = {{Contribution of mathematical modeling to the fight against bacterial antibiotic resistance}},
  AUTHOR = {Opatowski, Lulla and Guillemot, Didier and Bo{\"e}lle, Pierre-Yves and Temime, Laura},
  URL = {https://hal-cnam.archives-ouvertes.fr/hal-02089219},
  JOURNAL = {{Current Opinion in Infectious Diseases}},
  PUBLISHER = {{Lippincott, Williams \& Wilkins}},
  VOLUME = {24},
  NUMBER = {3},
  PAGES = {279-287},
  YEAR = {2011},
  DOI = {10.1097/QCO.0b013e3283462362},
}
@article{article6,
author = {Martcheva, M.},
year = {2015},
month = {01},
pages = {},
title = {An Introduction to Mathematical Epidemiology},
volume = {61},
isbn = {978-1-4899-7611-6},
doi = {10.1007/978-1-4899-7612-3}
}
@article{Siettos2013,
title = {Mathematical modeling of infectious disease dynamics},
journal = {Virulence},
volume = {4},
pages = {295-306},
year = {2013},
doi = {https://doi:10.4161/viru.24041},
author = {Siettos, Constantinos I, and Lucia Russo},
}
@article{Keeling2009,
 author = {Keeling, M. J. and Danon, L.},
 title = "{Mathematical modelling of infectious diseases}",
 journal = {British Medical Bulletin},
 volume = {92},
 number = {1},
 pages = {33-42},
 year = {2009},
 month = {10},
 issn = {0007-1420},
 doi = {10.1093/bmb/ldp038},
 url = {https://doi.org/10.1093/bmb/ldp038},
 eprint = {https://academic.oup.com/bmb/article-pdf/92/1/33/954051/ldp038.pdf},
}

@article{BURTON201291,
title = {Disease persistence in epidemiological models: The interplay between vaccination and migration},
journal = {Mathematical Biosciences},
volume = {239},
number = {1},
pages = {91-96},
year = {2012},
issn = {0025-5564},
doi = {https://doi.org/10.1016/j.mbs.2012.05.003},
url = {https://www.sciencedirect.com/science/article/pii/S0025556412001198},
author = {Jackson Burton and Lora Billings and Derek A.T. Cummings and Ira B. Schwartz},
}

@article{Grassly2008,
title = {Mathematical models of infectious disease transmission},
journal = {Nat Rev Microbiol},
volume = {6},
pages = {477-487},
year = {2008},
doi = {https://doi: 10.1038/nrmicro1845},
author = {Grassly NC, Fraser C.},
}
@article{ALLEN2017128,
title = {A primer on stochastic epidemic models: Formulation, numerical simulation, and analysis},
journal = {Infectious Disease Modelling},
volume = {2},
number = {2},
pages = {128-142},
year = {2017},
issn = {2468-0427},
doi = {https://doi.org/10.1016/j.idm.2017.03.001},
url = {https://www.sciencedirect.com/science/article/pii/S2468042716300495},
author = {Linda J.S. Allen},
}
@article{Wang2020,
author = {Wang, Xiaodong and Wang, Chunxia and Wang, Kai},
year = {2020},
month = {12},
pages = {},
title = {Global dynamics of a novel deterministic and stochastic SIR epidemic model with vertical transmission and media coverage},
volume = {2020},
journal = {Advances in Difference Equations},
doi = {10.1186/s13662-020-03145-3}
}
@article{Funk2010,
author = {Funk, Sebastian and Salathé, Marcel and Jansen, Vincent},
year = {2010},
month = {09},
pages = {1247-56},
title = {Modelling the Influence of Human Behaviour on the Spread of Infectious Diseases: A Review},
volume = {7},
journal = {Journal of the Royal Society, Interface / the Royal Society},
doi = {10.1098/rsif.2010.0142}
}
@article{Emerenini2017,
author = {Emerenini, Blessing and Inyama, Simeon},
year = {2017},
month = {10},
pages = {},
title = {Mathematical Model and Analysis of Transmission Dynamics of Hepatitis B Virus},
volume = {7},
journal = {F1000Research},
doi = {10.12688/f1000research.15557.1}
}
@article{naresh2009stability,
  title={Stability analysis of a time delayed SIR epidemic model with nonlinear incidence rate},
  author={Naresh, Ram and Tripathi, Agraj and Tchuenche, Jean M and Sharma, Dileep},
  journal={Computers \& mathematics with applications},
  volume={58},
  number={2},
  pages={348--359},
  year={2009},
  publisher={Elsevier}
}
@article{And1,
author = {Omame, Andrew and Sene, Ndolane and Nometa, Ikenna and Nwakanma, Cosmas and Nwafor, Emmanuel and Iheonu, Nneka and Daniel, Okuonghae},
year = {2021},
month = {11},
pages = {1568-1590},
title = {Analysis of COVID-19 and comorbidity co-infection model with optimal control},
volume = {42},
journal = {Optimal Control Applications and Methods},
doi = {10.1002/oca.2748}
}

@article{article3,
author = {Dreessche, P and Watmough, James},
year = {2002},
month = {11},
pages = {29-48},
title = {Reproduction Numbers and Sub-threshold Endemic Equilibria for Compartmental Models of Disease Transmission},
volume = {180},
journal = {Mathematical Biosciences},
doi = {10.1016/S0025-5564(02)00108-6}
}
@article{article,
author = {Hattaf, Khalid and Dutta, Hemen},
year = {2020},
month = {07},
pages = {109916},
title = {Modeling the dynamics of viral infections in presence of latently infected cells},
volume = {136},
journal = {Chaos Solitons \& Fractals},
doi = {10.1016/j.chaos.2020.109916}
}
@article{DONOFRIO2022112072,
title = {Behavioral SIR models with incidence-based social-distancing},
journal = {Chaos, Solitons \& Fractals},
volume = {159},
pages = {112072},
year = {2022},
issn = {0960-0779},
doi = {https://doi.org/10.1016/j.chaos.2022.112072},
url = {https://www.sciencedirect.com/science/article/pii/S096007792200282X},
author = {Alberto d'Onofrio and Piero Manfredi},
}
@article{Singh_2022,
doi = {10.1088/1742-6596/2267/1/012011},
url = {https://dx.doi.org/10.1088/1742-6596/2267/1/012011},
year = {2022},
month = {may},
publisher = {IOP Publishing},
volume = {2267},
number = {1},
pages = {012011},
author = {Raminder Pal Singh},
title = {Bifurcation and Stability Analysis of Delayed SIR Model},
journal = {Journal of Physics: Conference Series},
}
@article{article5,
author = {Elazzouzi, Abdelhai and Abdesslem, Lamrani and Tilioua, Mouhcine and Tridane, Abdessamad},
year = {2019},
month = {12},
pages = {},
title = {Global stability analysis for a generalized delayed SIR model with vaccination and treatment},
volume = {2019},
journal = {Advances in Difference Equations},
doi = {10.1186/s13662-019-2447-z}
}
@book{liao2007stability,
  title={Stability of Dynamical Systems},
  author={Liao, X. and Wang, L.Q. and Yu, P.},
  isbn={9780080550619},
  series={ISSN},
  url={https://books.google.co.in/books?id=sKPYmdrEtKEC},
  year={2007},
  publisher={Elsevier Science}
}
@article{comparisonthm1,
author = {Li, Wenjie and Ji, J.C. and Lihong, Huang},
year = {2020},
month = {06},
pages = {1},
title = {Dynamics of a discontinuous computer worm system},
volume = {148},
journal = {Proceedings of the American Mathematical Society},
doi = {10.1090/proc/15095}
}
@article{WINTACHAI2021e06812,
title = {Stability analysis of SEIR model related to efficiency of vaccines for COVID-19 situation},
journal = {Heliyon},
volume = {7},
number = {4},
pages = {e06812},
year = {2021},
issn = {2405-8440},
doi = {https://doi.org/10.1016/j.heliyon.2021.e06812},
url = {https://www.sciencedirect.com/science/article/pii/S2405844021009154},
author = {Phitchayapak Wintachai and Kiattisak Prathom},
}
Values = https://www.tn.data.gov.in/catalog/covid-19].
@article{dickson2022sqirv,
  title={SQIRV MODEL FOR OMICRON VARIANT WITH TIME DELAY},
  author={dickson, S and Padmasekaran, S and Chatzarakis, GE and Panetsos, SL},
  journal={J. Math. Anal. Appl},
  volume={19},
  number={2},
  year={2022}
}
@article{zaman2017optimal,
  title={Optimal strategy of vaccination \& treatment in an SIR epidemic model},
  author={Zaman, Gul and Kang, Yong Han and Cho, Giphil and Jung, Il Hyo},
  journal={Mathematics and computers in simulation},
  volume={136},
  pages={63--77},
  year={2017},
  publisher={Elsevier}
}
@article{saha2022dynamical,
  title={Dynamical behavior of SIRS model incorporating government action and public response in presence of deterministic and fluctuating environments},
  author={Saha, Sangeeta and Dutta, Protyusha and Samanta, Guruprasad},
  journal={Chaos, Solitons \& Fractals},
  volume={164},
  pages={112643},
  year={2022},
  publisher={Elsevier}
}
@article{BEKIROS2020109828,
title = {SBDiEM: A new mathematical model of infectious disease dynamics},
journal = {Chaos, Solitons \& Fractals},
volume = {136},
pages = {109828},
year = {2020},
issn = {0960-0779},
doi = {https://doi.org/10.1016/j.chaos.2020.109828},
url = {https://www.sciencedirect.com/science/article/pii/S0960077920302289},
author = {Stelios Bekiros and Dimitra Kouloumpou},
}
@article{HATTAF2020109916,
title = {Modeling the dynamics of viral infections in presence of latently infected cells},
journal = {Chaos, Solitons \& Fractals},
volume = {136},
pages = {109916},
year = {2020},
issn = {0960-0779},
doi = {https://doi.org/10.1016/j.chaos.2020.109916},
url = {https://www.sciencedirect.com/science/article/pii/S0960077920303167},
author = {Khalid Hattaf and Hemen Dutta},
}
@article{wintachai2021stability,
  title={Stability analysis of SEIR model related to efficiency of vaccines for COVID-19 situation},
  author={Wintachai, Phitchayapak and Prathom, Kiattisak},
  journal={Heliyon},
  volume={7},
  number={4},
  pages={e06812},
  year={2021},
  publisher={Elsevier}
}
@article{kabir2019analysis,
  title={Analysis of SIR epidemic model with information spreading of awareness},
  author={Kabir, KM Ariful and Kuga, Kazuki and Tanimoto, Jun},
  journal={Chaos, Solitons \& Fractals},
  volume={119},
  pages={118--125},
  year={2019},
  publisher={Elsevier}
}
@article{ali2020analysis,
  title={Analysis of stochastic delayed SIRS model with exponential birth and saturated incidence rate},
  author={Ali, Ishtiaq and Khan, Sami Ullah},
  journal={Chaos, Solitons \& Fractals},
  volume={138},
  pages={110008},
  year={2020},
  publisher={Elsevier}
}
@article{cooper2020sir,
  title={A SIR model assumption for the spread of COVID-19 in different communities},
  author={Cooper, Ian and Mondal, Argha and Antonopoulos, Chris G},
  journal={Chaos, Solitons \& Fractals},
  volume={139},
  pages={110057},
  year={2020},
  publisher={Elsevier}
}
Scopus
EXPORT DATE: 06 June 2023

@ARTICLE{Kermack1927700,
	author = {Kermack, W.O. and McKendrick, A.G. and Walker, G.T.},
        title = {A contribution to the mathematical theory of epidemics},
        journal = {Proc. R. Soc. Lond. A},
 year = {1927},
	pages = {700 – 721},
	url = {https://www.scopus.com/inward/record.uri?eid=2-s2.0-85124422199\&partnerID=40\&md5=3365673d9b6965b0c09dc482a964eb08},
	type = {Article},
	publication_stage = {Final},
	source = {Scopus},
	note = {Cited by: 1}
}
Scopus
EXPORT DATE: 06 June 2023

@ARTICLE{Bernoulli17601,
title={Daniel Bernoulli, d'Alembert and the inoculation of smallpox (1760)},
	author = {Bernoulli, D.},
	year = {1760},
	journal = {Mm. Des Math. Et Phys., Mem},
	pages = {1},
	url = {https://www.scopus.com/inward/record.uri?eid=2-s2.0-85093183258\&partnerID=40\&md5=133db245d2580e4f23f2f0ae530fd4ae},
	type = {Article},
	publication_stage = {Final},
	source = {Scopus},
	note = {Cited by: 0}
}
@book{hamer1906epidemic,
  title={Epidemic disease in England: the evidence of variability and of persistency of type},
  author={Hamer, William Heaton},
  year={1906},
  publisher={Bedford Press}
}
@article{li1995global,
  title={Global stability for the SEIR model in epidemiology},
  author={Li, Michael Y and Muldowney, James S},
  journal={Mathematical biosciences},
  volume={125},
  number={2},
  pages={155--164},
  year={1995},
  publisher={Elsevier}
}
@article{dantas2018calibration,
  title={Calibration of a SEIR--SEI epidemic model to describe the Zika virus outbreak in Brazil},
  author={Dantas, Eber and Tosin, Michel and Cunha Jr, Americo},
  journal={Applied Mathematics and Computation},
  volume={338},
  pages={249--259},
  year={2018},
  publisher={Elsevier}
}
@article{ZHANG20081456,
title = {Global asymptotic stability of a delayed SEIRS epidemic model with saturation incidence},
journal = {Chaos, Solitons \& Fractals},
volume = {37},
number = {5},
pages = {1456-1468},
year = {2008},
issn = {0960-0779},
doi = {https://doi.org/10.1016/j.chaos.2006.10.041},
url = {https://www.sciencedirect.com/science/article/pii/S0960077906010071},
author = {Tailei Zhang and Zhidong Teng},
}
@article{WANG20102390,
title = {Analysis of an SIR model with bilinear incidence rate},
journal = {Nonlinear Analysis: Real World Applications},
volume = {11},
number = {4},
pages = {2390-2402},
year = {2010},
issn = {1468-1218},
doi = {https://doi.org/10.1016/j.nonrwa.2009.07.012},
url = {https://www.sciencedirect.com/science/article/pii/S1468121809002430},
author = {Jian-Jun Wang and Jin-Zhu Zhang and Zhen Jin},
keywords = {SIR model, Time delay, Stability, Hopf bifurcation},
}
